DRL-STNet: Unsupervised Domain Adaptation for Cross-modality Medical Image Segmentation via Disentangled Representation Learning

Unsupervised domain adaptation (UDA) is essential for medical image segmentation, especially in cross-modality data scenarios. UDA aims to transfer knowledge from a labeled source domain to an unlabeled target domain, thereby reducing the dependency on extensive manual annotations. This paper presents DRL-STNet, a novel framework for cross-modality medical image segmentation that leverages generative adversarial networks (GANs), disentangled representation learning (DRL), and self-training (ST). Our method leverages DRL within a GAN to translate images from the source to the target modality. Then, the segmentation model is initially trained with these translated images and corresponding source labels and then fine-tuned iteratively using a combination of synthetic and real images with pseudo-labels and real labels. The proposed framework exhibits superior performance in abdominal organ segmentation on the FLARE challenge dataset, surpassing state-of-the-art methods by 11.4% in the Dice similarity coefficient and by 13.1% in the Normalized Surface Dice metric, achieving scores of 74.21% and 80.69%, respectively. The average running time is 41 seconds, and the area under the GPU memory-time curve is 11,292 MB. These results indicate the potential of DRL-STNet for enhancing cross-modality medical image segmentation tasks.

==> ref.tex <==
@article{simpson2019MSD,
author = {Amber L. Simpson and Michela Antonelli and Spyridon Bakas and Michel Bilello and Keyvan Farahani and Bram van Ginneken and Annette Kopp-Schneider and Bennett A. Landman and Geert Litjens and Bjoern Menze and Olaf Ronneberger and Ronald M. Summers and Patrick Bilic and Patrick F. Christ and Richard K. G. Do and Marc Gollub and Jennifer Golia-Pernicka and Stephan H. Heckers and William R. Jarnagin and Maureen K. McHugo and Sandy Napel and Eugene Vorontsov and Lena Maier-Hein and M. Jorge Cardoso},
title = {A large annotated medical image dataset for the development and evaluation of segmentation algorithms},
year = {2019},
journal = {arXiv preprint arXiv:1902.09063},
}



@article{KiTS,
title = {The state of the art in kidney and kidney tumor segmentation in contrast-enhanced CT imaging: Results of the KiTS19 challenge},
journal = {Medical Image Analysis},
volume = {67},
pages = {101821},
year = {2021},
author = {Nicholas Heller and Fabian Isensee and Klaus H. Maier-Hein and Xiaoshuai Hou and Chunmei Xie and Fengyi Li and Yang Nan and Guangrui Mu and Zhiyong Lin and Miofei Han and Guang Yao and Yaozong Gao and Yao Zhang and Yixin Wang and Feng Hou and Jiawei Yang and Guangwei Xiong and Jiang Tian and Cheng Zhong and Jun Ma and Jack Rickman and Joshua Dean and Bethany Stai and Resha Tejpaul and Makinna Oestreich and Paul Blake and Heather Kaluzniak and Shaneabbas Raza and Joel Rosenberg and Keenan Moore and Edward Walczak and Zachary Rengel and Zach Edgerton and Ranveer Vasdev and Matthew Peterson and Sean McSweeney and Sarah Peterson and Arveen Kalapara and Niranjan Sathianathen and Nikolaos Papanikolopoulos and Christopher Weight}
}


@article{KiTSDataset,
  title={An international challenge to use artificial intelligence to define the state-of-the-art in kidney and kidney tumor segmentation in CT imaging.},
  author={Heller, Nicholas and McSweeney, Sean and Peterson, Matthew Thomas and Peterson, Sarah and Rickman, Jack and Stai, Bethany and Tejpaul, Resha and Oestreich, Makinna and Blake, Paul and Rosenberg, Joel and others},
  volume = {38},
  number = {6},
  pages = {626-626},
  year = {2020},
  journal={American Society of Clinical Oncology}
}


@article{AMOS,
  title={Amos: A large-scale abdominal multi-organ benchmark for versatile medical image segmentation},
  author={Ji, Yuanfeng and Bai, Haotian and GE, Chongjian and Yang, Jie and Zhu, Ye and Zhang, Ruimao and Li, Zhen and Zhanng, Lingyan and Ma, Wanling and Wan, Xiang and Luo, Ping},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={36722--36732},
  year={2022}
}

@article{LLD-MMRI,
      title={SDR-Former: A Siamese Dual-Resolution Transformer for Liver Lesion Classification Using 3D Multi-Phase Imaging}, 
      author={Meng Lou and Hanning Ying and Xiaoqing Liu and Hong-Yu Zhou and Yuqing Zhang and Yizhou Yu},
      journal={arXiv preprint arXiv:2402.17246},
      year={2024}
}


@inproceedings{U-Net,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={International Conference on Medical image computing and computer-assisted intervention},
  pages={234--241},
  year={2015}
}

@article{AbdomenCT-1K,
  title={AbdomenCT-1K: Is Abdominal Organ Segmentation A Solved Problem?},
  author={Ma, Jun and Zhang, Yao and Gu, Song and Zhu, Cheng and Ge, Cheng and Zhang, Yichi and An, Xingle and Wang, Congcong and Wang, Qiyuan and Liu, Xin and Cao, Shucheng and Zhang, Qi and Liu, Shangqing and Wang, Yunpeng and Li, Yuhui and He, Jian and Yang, Xiaoping},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={44},
  number={10},
  pages={6695-6714},
  year={2022}
}


@article{MedIA-FLARE21,
title = {Fast and Low-GPU-memory abdomen CT organ segmentation: The FLARE challenge},
author = {Jun Ma and Yao Zhang and Song Gu and Xingle An and Zhihe Wang and Cheng Ge and Congcong Wang and Fan Zhang and Yu Wang and Yinan Xu and Shuiping Gou and Franz Thaler and Christian Payer and Darko Štern and Edward G.A. Henderson and Dónal M. McSweeney and Andrew Green and Price Jackson and Lachlan McIntosh and Quoc-Cuong Nguyen and Abdul Qayyum and Pierre-Henri Conze and Ziyan Huang and Ziqi Zhou and Deng-Ping Fan and Huan Xiong and Guoqiang Dong and Qiongjie Zhu and Jian He and Xiaoping Yang},
journal = {Medical Image Analysis},
volume = {82},
pages = {102616},
year = {2022}
}

@inproceedings{FLARE22-1st-Huang,
  title={Revisiting nnU-net for iterative pseudo labeling and efficient sliding window inference},
  author={Huang, Ziyan and Wang, Haoyu and Ye, Jin and Niu, Jingqi and Tu, Can and Yang, Yuncheng and Du, Shiyi and Deng, Zhongying and Gu, Lixu and He, Junjun},
  booktitle={MICCAI Challenge on Fast and Low-Resource Semi-supervised Abdominal Organ Segmentation},
  pages={178--189},
  year={2022},
  publisher={Springer}
}

@inproceedings{FLARE22-bestDSC-Wang,
  title={Cascade dual-decoders network for abdominal organs segmentation},
  author={Wang, Ershuai and Zhao, Yaliang and Wu, Yajun},
  booktitle={MICCAI Challenge on Fast and Low-Resource Semi-supervised Abdominal Organ Segmentation},
  pages={202--213},
  year={2022},
  publisher={Springer},
}

@incollection{FLARE23-1st,
  title={Fast abdomen organ and tumor segmentation with nn-UNet},
  author={Wu, Yajun and Wang, Ershuai and Shao, Zhenzhou},
  booktitle={MICCAI Challenge on Fast and Low-Resource Semi-supervised Abdominal Organ Segmentation},
  pages={1--14},
  year={2023},
  publisher={Springer}
}

@article{FLARE22,
    author = {Jun Ma and Yao Zhang and Song Gu and Cheng Ge and Shihao Ma and Adamo Young and Cheng Zhu and Kangkang Meng and Xin Yang and Ziyan Huang and Fan Zhang and Wentao Liu and YuanKe Pan and Shoujin Huang and Jiacheng Wang and Mingze Sun and Weixin Xu and Dengqiang Jia and Jae Won Choi and Natália Alves and Bram de Wilde and Gregor Koehler and Yajun Wu and Manuel Wiesenfarth and Qiongjie Zhu and Guoqiang Dong and Jian He and the FLARE Challenge Consortium and Bo Wang},
    title = {Unleashing the Strengths of Unlabeled Data in Pan-cancer Abdominal Organ Quantification: the FLARE22 Challenge},
    year = {2024},
    journal = {Lancet Digital Health},
}

@article{FLARE23,
Author = {Jun Ma and Yao Zhang and Song Gu and Cheng Ge and Ershuai Wang and Qin Zhou and Ziyan Huang and Pengju Lyu and Jian He and Bo Wang},
Title = {Automatic Organ and Pan-cancer Segmentation in Abdomen CT: the FLARE 2023 Challenge},
Year = {2024},
journal = {arXiv preprint arXiv:2408.12534},
}

@article{SAM2,
Author = {Nikhila Ravi and Valentin Gabeur and Yuan-Ting Hu and Ronghang Hu and Chaitanya Ryali and Tengyu Ma and Haitham Khedr and Roman Rädle and Chloe Rolland and Laura Gustafson and Eric Mintun and Junting Pan and Kalyan Vasudev Alwala and Nicolas Carion and Chao-Yuan Wu and Ross Girshick and Piotr Dollár and Christoph Feichtenhofer},
Title = {SAM 2: Segment Anything in Images and Videos},
Year = {2024},
journal = {arXiv:2408.00714},
}



@article{MedSAM,
  title={Segment anything in medical images},
  author={Ma, Jun and He, Yuting and Li, Feifei and Han, Lin and You, Chenyu and Wang, Bo},
  journal={Nature Communications},
  volume={15},
  pages={654},
  year={2024}
}

@article{MedSAM2,
  title={Segment Anything in Medical Images and Videos: Benchmark and Deployment},
  author={Ma, Jun and Kim, Sumin and Li, Feifei and Baharoon, Mohammed and Asakereh, Reza and Lyu, Hongwei and Wang, Bo},
  journal={arXiv preprint arXiv:2408.03322},
  year={2024}
}


@article{nnUNet,
  title={nnU-Net: a self-configuring method for deep learning-based biomedical image segmentation},
  author={Isensee, Fabian and Jaeger, Paul F and Kohl, Simon AA and Petersen, Jens and Maier-Hein, Klaus H},
  journal={Nature Methods},
  volume={18},
  number={2},
  pages={203--211},
  year={2021}
}

@article{LossOdyssey,
title = {Loss Odyssey in Medical Image Segmentation},
journal = {Medical Image Analysis},
volume = {71},
pages = {102035},
year = {2021},
author = {Jun Ma and Jianan Chen and Matthew Ng and Rui Huang and Yu Li and Chen Li and Xiaoping Yang and Anne L. Martel}
}


@article{LiTS,
    title = {The Liver Tumor Segmentation Benchmark (LiTS)},
    journal = {Medical Image Analysis},
    volume = {84},
    pages = {102680},
    year = {2023},
    author = {Patrick Bilic and Patrick Christ and Hongwei Bran Li and Eugene Vorontsov and Avi Ben-Cohen and Georgios Kaissis and Adi Szeskin and Colin Jacobs and Gabriel Efrain Humpire Mamani and Gabriel Chartrand and Fabian Lohöfer and Julian Walter Holch and Wieland Sommer and Felix Hofmann and Alexandre Hostettler and Naama Lev-Cohain and Michal Drozdzal and Michal Marianne Amitai and Refael Vivanti and Jacob Sosna and Ivan Ezhov and Anjany Sekuboyina and Fernando Navarro and Florian Kofler and Johannes C. Paetzold and Suprosanna Shit and Xiaobin Hu and Jana Lipková and Markus Rempfler and Marie Piraud and Jan Kirschke and Benedikt Wiestler and Zhiheng Zhang and Christian Hülsemeyer and Marcel Beetz and Florian Ettlinger and Michela Antonelli and Woong Bae and Míriam Bellver and Lei Bi and Hao Chen and Grzegorz Chlebus and Erik B. Dam and Qi Dou and Chi-Wing Fu and Bogdan Georgescu and Xavier Giró-i-Nieto and Felix Gruen and Xu Han and Pheng-Ann Heng and Jürgen Hesser and Jan Hendrik Moltz and Christian Igel and Fabian Isensee and Paul Jäger and Fucang Jia and Krishna Chaitanya Kaluva and Mahendra Khened and Ildoo Kim and Jae-Hun Kim and Sungwoong Kim and Simon Kohl and Tomasz Konopczynski and Avinash Kori and Ganapathy Krishnamurthi and Fan Li and Hongchao Li and Junbo Li and Xiaomeng Li and John Lowengrub and Jun Ma and Klaus Maier-Hein and Kevis-Kokitsi Maninis and Hans Meine and Dorit Merhof and Akshay Pai and Mathias Perslev and Jens Petersen and Jordi Pont-Tuset and Jin Qi and Xiaojuan Qi and Oliver Rippel and Karsten Roth and Ignacio Sarasua and Andrea Schenk and Zengming Shen and Jordi Torres and Christian Wachinger and Chunliang Wang and Leon Weninger and Jianrong Wu and Daguang Xu and Xiaoping Yang and Simon Chun-Ho Yu and Yading Yuan and Miao Yue and Liping Zhang and Jorge Cardoso and Spyridon Bakas and Rickmer Braren and Volker Heinemann and Christopher Pal and An Tang and Samuel Kadoury and Luc Soler and Bram {van Ginneken} and Hayit Greenspan and Leo Joskowicz and Bjoern Menze},
}


@article{TotalSegmentator,
author = {Wasserthal, Jakob and Breit, Hanns-Christian and Meyer, Manfred T. and Pradella, Maurice and Hinck, Daniel and Sauter, Alexander W. and Heye, Tobias and Boll, Daniel T. and Cyriac, Joshy and Yang, Shan and Bach, Michael and Segeroth, Martin},
title = {TotalSegmentator: Robust Segmentation of 104 Anatomic Structures in CT Images},
journal = {Radiology: Artificial Intelligence},
volume = {5},
number = {5},
pages = {e230024},
year = {2023}
}

@article{autoPET-Data,
  title={A whole-body FDG-PET/CT Dataset with manually annotated Tumor Lesions},
  author={Gatidis, Sergios and Hepp, Tobias and Fr{\"u}h, Marcel and La Foug{\`e}re, Christian and Nikolaou, Konstantin and Pfannenberg, Christina and Sch{\"o}lkopf, Bernhard and K{\"u}stner, Thomas and Cyran, Clemens and Rubin, Daniel},
  journal={Scientific Data},
  volume={9},
  number={1},
  pages={601},
  year={2022}
}

@article{autoPET-MICCAI22,
  title={The autoPET challenge: Towards fully automated lesion segmentation in oncologic PET/CT imaging},
  author={Gatidis, Sergios and Fr{\"u}h, Marcel and Fabritius, Matthias and Gu, Sijing and Nikolaou, Konstantin and La Foug{\`e}re, Christian and Ye, Jin and He, Junjun and Peng, Yige and Bi, Lei and others},
  journal={preprint at Research Square (Nature Portfolio )},
  doi={https://doi.org/10.21203/rs.3.rs-2572595/v1},
  year={2023}
}


@article{TCIA,
  title={The Cancer Imaging Archive (TCIA): maintaining and operating a public information repository},
  author={Clark, Ken and Vendt, Bruce and Smith, Kirk and Freymann, John and Kirby, Justin and Koppel, Paul and Moore, Stephen and Phillips, Stephen and Maffitt, Derek and Pringle, Michael and Tarbox, Lawrence and Prior, Fred},
  journal={Journal of Digital Imaging},
  volume={26},
  number={6},
  pages={1045--1057},
  year={2013}
}

@inproceedings{ITKSNAP,
  title={ITK-SNAP: An interactive tool for semi-automatic segmentation of multi-modality biomedical images},
  author={Yushkevich, Paul A and Gao, Yang and Gerig, Guido},
  booktitle={Annual International Conference of the IEEE Engineering in Medicine and Biology Society},
  pages={3342--3345},
  year={2016}
}

@article{Slicer,
  title={3D Slicer as an image computing platform for the Quantitative Imaging Network},
  author={Fedorov, Andriy and Beichel, Reinhard and Kalpathy-Cramer, Jayashree and Finet, Julien and Fillion-Robin, Jean-Christophe and Pujol, Sonia and Bauer, Christian and Jennings, Dominique and Fennessy, Fiona and Sonka, Milan and others},
  journal={Magnetic Resonance Imaging},
  volume={30},
  number={9},
  pages={1323--1341},
  year={2012}
}

@article{codabench,
    title = {Codabench: Flexible, easy-to-use, and reproducible meta-benchmark platform},
    author = {Zhen Xu and Sergio Escalera and Adrien Pavão and Magali Richard and Wei-Wei Tu and Quanming Yao and Huan Zhao and Isabelle Guyon},
    journal = {Patterns},
    volume = {3},
    number = {7},
    pages = {100543},
    year = {2022}
} 

@article{wang2018deep,
  title={Deep visual domain adaptation: A survey},
  author={Wang, Mei and Deng, Weihong},
  journal={Neurocomputing},
  volume={312},
  pages={135--153},
  year={2018},
  publisher={Elsevier}
}

@article{liu2021review,
  title={A review of deep-learning-based medical image segmentation methods},
  author={Liu, Xiangbin and Song, Liping and Liu, Shuai and Zhang, Yudong},
  journal={Sustainability},
  volume={13},
  number={3},
  pages={1224},
  year={2021},
  publisher={MDPI}
}

@article{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Advances in neural information processing systems},
  volume={27},
  year={2014}
}

@article{bengio2013representation,
  title={Representation learning: A review and new perspectives},
  author={Bengio, Yoshua and Courville, Aaron and Vincent, Pascal},
  journal={IEEE Transactions on pattern analysis and machine intelligence},
  volume={35},
  number={8},
  pages={1798--1828},
  year={2013},
  publisher={IEEE}
}

@inproceedings{Shi2021A,
  title={A multi-task unsupervised domain adaptation network for medical image segmentation},
  author={Shi, Yuejing and Zhu, Fan and Peng, Yan and Ye, Zhen and Zhou, Chaozheng},
  booktitle={International Conference on Image Processing and Intelligent Control (IPIC 2021)},
  volume={11928},
  pages={65--70},
  year={2021},
  organization={SPIE}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}
@inproceedings{mao2017least,
  title={Least squares generative adversarial networks},
  author={Mao, Xudong and Li, Qing and Xie, Haoran and Lau, Raymond YK and Wang, Zhen and Paul Smolley, Stephen},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2794--2802},
  year={2017}
}

@article{Yao2022A,title={A Novel 3D Unsupervised Domain Adaptation Framework for Cross-Modality Medical Image Segmentation},author={Kai Yao and Zixian Su and Kaizhu Huang and Xi Yang and Jie Sun and A. Hussain and Frans Coenen},journal={IEEE Journal of Biomedical and Health Informatics},year={2022},volume={26},pages={4976-4986},doi={10.1109/JBHI.2022.3162118}
}

@INPROCEEDINGS{lin2024brighteye,
  author={Lin, Hui and Apostolidis, Charilaos and Katsaggelos, Aggelos K.},
  booktitle={2024 IEEE International Symposium on Biomedical Imaging (ISBI)}, 
  title={Brighteye: Glaucoma Screening with Color Fundus Photographs Based on Vision Transformer}, 
  year={2024},
  volume={},
  number={},
  pages={1-4},
  keywords={Glaucoma;Computer vision;Biomedical optical imaging;Sensitivity;Image color analysis;Transformers;Optical imaging;Glaucoma screening;color fundus photography;optic disc detection;vision transformer;feature aggregation;image classification},
  doi={10.1109/ISBI56570.2024.10635883}}

@article{lin2023stenunet,
  title={StenUNet: Automatic Stenosis Detection from X-ray Coronary Angiography},
  author={Lin, Hui and Liu, Tom and Katsaggelos, Aggelos and Kline, Adrienne},
  journal={arXiv preprint arXiv:2310.14961},
  year={2023}
}

@article{Wu2021Unsupervised,
title={Unsupervised Domain Adaptation With Variational Approximation for Cardiac Segmentation},
author={Fuping Wu and X. Zhuang},
journal={IEEE Transactions on Medical Imaging},
year={2021},
volume={40},
pages={3555-3567},
doi={10.1109/TMI.2021.3090412}
}

@inproceedings{schiffers2018synthetic,
  title={Synthetic fundus fluorescein angiography using deep neural networks},
  author={Schiffers, Florian and Yu, Zekuan and Arguin, Steve and Maier, Andreas and Ren, Qiushi},
  booktitle={Bildverarbeitung f{\"u}r die Medizin 2018: Algorithmen-Systeme-Anwendungen. Proceedings des Workshops vom 11. bis 13. M{\"a}rz 2018 in Erlangen},
  pages={234--238},
  year={2018},
  organization={Springer}
}


@article{song2020denoising,
  title={Denoising diffusion implicit models},
  author={Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
  journal={arXiv preprint arXiv:2010.02502},
  year={2020}
}

@article{chen2020unsupervised,title={Unsupervised Bidirectional Cross-Modality Adaptation via Deeply Synergistic Image and Feature Alignment for Medical Image Segmentation},author={Cheng Chen and Q. Dou and Hao Chen and J. Qin and P. Heng},journal={IEEE Transactions on Medical Imaging},year={2020},volume={39},pages={2494-2505},doi={10.1109/TMI.2020.2972701}
}


@article{Xie2022Unsupervised,title={Unsupervised Domain Adaptation for Medical Image Segmentation by Disentanglement Learning and Self-Training.},author={Qingsong Xie and Yuexiang Li and Nanjun He and Munan Ning and Kai Ma and Guoxing Wang and Yong Lian and Yefeng Zheng},journal={IEEE transactions on medical imaging},year={2022},volume={PP},doi={10.1109/TMI.2022.3192303}
}

@article{liu2017unsupervised,
  title={Unsupervised image-to-image translation networks},
  author={Liu, Ming-Yu and Breuel, Thomas and Kautz, Jan},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{zhu2017unpaired,
  title={Unpaired image-to-image translation using cycle-consistent adversarial networks},
  author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
  booktitle={Proceedings of the IEEE International Conference on computer vision},
  pages={2223--2232},
  year={2017}
}


@article{lin2024usformer,
  title={Usformer: A Small Network for Left Atrium Segmentation of 3D LGE MRI},
  author={Lin, Hui and L{\'o}pez-Tapia, Santiago and Schiffers, Florian and Wu, Yunan and Gunasekaran, Suvai and Hwang, Julia and Bishara, Dima and Kholmovski, Eugene and Elbaz, Mohammed and Passman, Rod S and others},
  journal={Heliyon},
  year = {2024},
  ISSN = {2405-8440},
  publisher={Elsevier}
}


@article{liu2023yolo,
  title={YOLO-Angio: An Algorithm for Coronary Anatomy Segmentation},
  author={Liu, Tom and Lin, Hui and Katsaggelos, Aggelos K and Kline, Adrienne},
  journal={arXiv preprint arXiv:2310.15898},
  year={2023}
}
@article{lin2019automated,
  title={Automated defect inspection of LED chip using deep convolutional neural network},
  author={Lin, Hui and Li, Bin and Wang, Xinggang and Shu, Yufeng and Niu, Shuanglong},
  journal={Journal of Intelligent Manufacturing},
  volume={30},
  pages={2525--2534},
  year={2019},
  publisher={Springer}
}

@inproceedings{lee2018diverse,
  title={Diverse image-to-image translation via disentangled representations},
  author={Lee, Hsin-Ying and Tseng, Hung-Yu and Huang, Jia-Bin and Singh, Maneesh and Yang, Ming-Hsuan},
  booktitle={Proceedings of the European Conference on computer vision (ECCV)},
  pages={35--51},
  year={2018}
}

@article{reinke2021common,
  title={Common limitations of image processing metrics: A picture story},
  author={Reinke, Annika and Tizabi, Minu D and Sudre, Carole H and Eisenmann, Matthias and R{\"a}dsch, Tim and Baumgartner, Michael and Acion, Laura and Antonelli, Michela and Arbel, Tal and Bakas, Spyridon and others},
  journal={arXiv preprint arXiv:2104.05642},
  year={2021}
}
@inproceedings{shin2023sdc,
  title={SDC-UDA: volumetric unsupervised domain adaptation framework for slice-direction continuous cross-modality medical image segmentation},
  author={Shin, Hyungseob and Kim, Hyeongyu and Kim, Sewon and Jun, Yohan and Eo, Taejoon and Hwang, Dosik},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7412--7421},
  year={2023}
}
@inproceedings{lee2013pseudo,
  title={Pseudo-label: The simple and efficient semi-supervised learning method for deep neural networks},
  author={Lee, Dong-Hyun and others},
  booktitle={Workshop on challenges in representation learning, ICML},
  volume={3},
  number={2},
  pages={896},
  year={2013},
  organization={Atlanta}
}
@article{jiang2022disentangled,
  title={Disentangled representation and cross-modality image translation based unsupervised domain adaptation method for abdominal organ segmentation},
  author={Jiang, Kaida and Quan, Li and Gong, Tao},
  journal={International Journal of Computer Assisted Radiology and Surgery},
  volume={17},
  number={6},
  pages={1101--1113},
  year={2022},
  publisher={Springer}
}
@article{ji2022amos,
  title={AMOS: A Large-Scale Abdominal Multi-Organ Benchmark for Versatile Medical Image Segmentation},
  author={Ji, Yuanfeng and Bai, Haotian and Yang, Jie and Ge, Chongjian and Zhu, Ye and Zhang, Ruimao and Li, Zhen and Zhang, Lingyan and Ma, Wanling and Wan, Xiang and others},
  journal={arXiv preprint arXiv:2206.08023},
  year={2022}
}
@article{lou2024sdrformer,
      title={SDR-Former: A Siamese Dual-Resolution Transformer for Liver Lesion Classification Using 3D Multi-Phase Imaging}, 
      author={Meng Lou and Hanning Ying and Xiaoqing Liu and Hong-Yu Zhou and Yuqing Zhang and Yizhou Yu},
      journal={arXiv preprint arXiv:2402.17246},
      year={2024}
}



@article{isensee2021nnu,
  title={nnU-Net: a self-configuring method for deep learning-based biomedical image segmentation},
  author={Isensee, Fabian and Jaeger, Paul F and Kohl, Simon AA and Petersen, Jens and Maier-Hein, Klaus H},
  journal={Nature methods},
  volume={18},
  number={2},
  pages={203--211},
  year={2021},
  publisher={Nature Publishing Group}
}
